Physical properties of three short period close binaries: kic 2715417, kic 6050116 and kic 6287172

We present the physical parameters of three short period close binaries using the observed data from Kepler Space Telescope. All of these observations were taken in a single bandpass (which approximates the Johnson V-band). Our three systems are KIC 2715417, KIC 6050116 and KIC 6287172. The first system KIC 2715417 is considered a semi-detached system with the secondary component filling the Roche lobe. The second system KIC 6050116 is an overcontact system, while the third system KIC 6287172 belongs to ellipsoidal variables (ELV) as deduced from the Roche lobe geometry. For photometric analysis, we used PHOEBE software package which is based on the Wilson-Devinney code (Wilson-Devinney 1971). Due to lack of spectroscopic data, the photometric mass ratios are determined from the analyses of the light curves using the Q-search method. The absolute parameters are determined using three different methods, Harmanec (1988), Maceroni-Van't Veer (1996) and Gazeas-Niarchos (2006).

==> bibtex.tex <==
@ARTICLE{Deb+etal+2010,
   author = {{Deb}, S. and {Singh}, H.~P. and {Seshadri}, T.~R. and {Gupta}, R.},
    title = "{A CCD photometric study of the late type contact binary EK Comae Berenices}",
  journal = {\ NewA},
  eprint = {arXiv:1004.5448},
 keywords = {binaries: close - stars : evolution - stars: individual EK Comae Berenices - stars: magnetic fields: spots},
     year = 2010,
    month = Nov,
   volume = 15,
    pages = {662-668},
      doi = {10.1016/j.newast.2010.04.005},
   url = {http://adsabs.harvard.edu/abs/2010NewA...15..662D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Drilling+Landolt+2002,
   author = {{Drilling}, J.~S. and {Landolt}, A.~U.},
    title = "{Allen's Astrophysical Quantities}",
  journal = {\ Normal Stars. In: Cox A.N. (eds) Allen's Astrophysical Quantities. Springer, New York, NY},
  eprint = {ISBN:978-1-4612-7037-9},
 keywords = {White Dwarf - Stellar Atmosphere - Apparent Magnitude - Spectral Classis - Standard Star},
     year = 2002,
    pages = {381-396},
      doi = {10.1007/978-1-4612-1186-0},
   url = {https://link.springer.com/chapter/10.1007/978-1-4612-1186-0},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Gazeas+Niarchos+2006,
   author = {{Gazeas}, K.~D. and {Niarchos}, P.~G.},
    title = "{Masses and angular momenta of contact binary stars}",
  journal = {\ MNRAS},
  eprint = {	arXiv:astro-ph/0606715},
 keywords = {instrumentation: miscellaneous, infrared: general},
     year = 2006,
    month = July,
   volume = 370,
    pages = {L29-L32},
      doi = {10.1111/j.1745-3933.2006.00182.x},
   url = {http://adsabs.harvard.edu/abs/2006MNRAS.370L..29G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Gazeas+Stepien+2008,
   author = {{Gazeas}, K. and {Stepien}, K.},
    title = "{Angular momentum and mass evolution of contact binaries}",
  journal = {\ MNRAS},
   eprint = {arXiv:0803.0212},
 keywords = {catalogues, surveys, quasars: emission lines, quasars: general},
     year = 2008,
    month = Nov,
   volume = 390,
    pages = {1577-1586},
      doi = {10.1111/j.1365-2966.2008.13844.x},
   url = {http://adsabs.harvard.edu/abs/2008MNRAS.390.1577G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
  }

@ARTICLE{Harmanec+1998,
   author = {{Harmanec}, P.},
    title = "{Stellar masses and radii based on modern binary data}",
  journal = {\ BAICz},
   eprint = {ISSN 0004-6248},
 keywords = {Early Stars - Eclipsing Binary Stars - Stellar Mass - Stellar Rotation -  B Stars - Light Curve - Main Sequence Stars - Stellar Magnitude - Stellar Spectra -  Stellar Temperature},
     year = 1998,
    month = Dec,
   volume = 39,
    pages = {329-345},
   url = {http://adsabs.harvard.edu/abs/1988BAICz..39..329H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
  }

@ARTICLE{Lucy+1967,
   author = {{Lucy}, L.~B.},
    title = "{Gravity-Darkening for Stars with Convective Envelopes}",
  journal = {\ ZA},
 keywords = {W Ursae Majoris - gravity darkening - Von Zeipel},
     year = 1967,
    month = Jan,
   volume = 65,
    pages = {89-92},
   url = {http://adsabs.harvard.edu/abs/1967ZA.....65...89L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Lucy+Wilson+1979,
   author = {{Lucy}, L.~B. and {Wilson}, R.~E.},
    title = "{Observational tests of theories of contact binaries}",
  journal = {\ APJ},
 keywords = {Binary Stars - Stellar Models - Early Stars - Light Curve - Stellar Evolution - Stellar Mass - Thermodynamic Equilibrium},
     year = 1979,
    month = July,
   volume = 231,
    pages = {502-513},
      doi = {10.1086/157212},
   url = {http://adsabs.harvard.edu/abs/1979ApJ...231..502L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Maceroni+Van'tVeer+1996,
   author = {{Maceroni}, C. and {Van'tVeer}, F.},
    title = "{The properties of W Ursae Majoris contact binaries: new results and old problems.}",
  journal = {\ A\&A},
 keywords = {BINARIES: CLOSE - STARS: EVOLUTION - STARS: MASS LOSS},
     year = 1996,
    month = July,
   volume = 311,
    pages = {523-531},
   url = {http://adsabs.harvard.edu/abs/1996A%26A...311..523M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Mowlavi+etal+2012,
   author = {{Mowlavi}, N. and {Eggenberger}, P. and {Meynet}, G. and {Ekstrom}, S. and {Georgy}, C. and {Maeder}, A. and {Charbonnel}, C. and {, Eyer}, L. },
    title = "{Stellar mass and age determinations - I. Grids of stellar models from Z=0.006 to 0.04 and M=0.5 to 3.5 Msun}",
  journal = {\ A\&A},
   eprint = {arXiv:1201.3628},
 keywords = {Stars: evolution - Hertzsprung-Russell and C-M diagrams - Stars: fundamental parameters -  Stars: low-mass},
     year = 2012,
    month = May,
   volume = 541,
    pages = {A41},
      doi = {10.1051/0004-6361/201117749},
   url = {http://adsabs.harvard.edu/abs/2012A%26A...541A..41M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{O'Connell+1951,
   author = {{O'Connell}, D.~J. },
    title = "{The so-called periastron effect in close eclipsing binaries ; New variable stars (fifth list)}",
  journal = {\ PRCO},
 keywords = {periastron effect - close eclipsing binaries - variable stars},
     year = 1951,
    month = January,
   volume = 2,
    pages = {85-100},
   url = {http://articles.adsabs.harvard.edu/full/1951PRCO....2...85O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Popper+1980,
   author = {{Popper}, D.~M. },
    title = "{Stellar masses}",
  journal = {\ ARA\&A},
     year = 1980,
    month = Jan,
   volume = 18,
    pages = {115-164},
      doi = {10.1146/annurev.aa.18.090180.000555},
   url = {http://adsabs.harvard.edu/abs/1980ARA&A..18..115P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Prsa+Zwitter+2005,
   author = {{Prsa}, A. and {Zwitter}, T.},
    title = "{A Computational Guide to Physics of Eclipsing Binaries. Paper I. Demonstrations and Perspectives}",
  journal = {\ ApJ},
   eprint = {arXiv:astro-ph/0503361},
 keywords = {Stars: Binaries: Eclipsing - Methods: Data Analysis - Methods: Numerical - Stars: Fundamental Parameters},
     year = 2005,
    month = July,
   volume = 628,
    pages = {426-438},
      doi = {10.1086/430591},
   url = {http://adsabs.harvard.edu/abs/2005ApJ...628..426P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Reed+1998,
   author = {{Reed}, B.~C. },
    title = "{The Composite Observational-Theoretical HR Diagram}",
  journal = {\ JRASC},
     year = 1998,
    month = Feb,
   volume = 92,
    pages = {36},
   url = {http://adsabs.harvard.edu/abs/1998JRASC..92...36R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Rucinski+1969,
   author = {{Ruciński}, S.~M. },
    title = "{The Proximity Effects in Close Binary Systems. II. The Bolometric Reflection Effect for Stars with Deep Convective Envelopes}",
  journal = {\ AcA},
     year = 1969,
    month = Jan,
   volume = 19,
    pages = {245},
   url = {http://adsabs.harvard.edu/abs/1969AcA....19..245R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Schlafly+Finkbeiner+2011,
   author = {{Schlafly}, E.~F. and {Finkbeiner}, D.~P. },
    title = "{Measuring Reddening with Sloan Digital Sky Survey Stellar Spectra and Recalibrating SFD}",
  journal = {\ ApJ},
   eprint = {arXiv:1012.4804},
 keywords = {dust - extinction - Galaxy: stellar content - ISM: clouds},
     year = 2011,
    month = Aug,
   volume = 737,
    pages = {103},
      doi = {10.1088/0004-637X/737/2/103},
   url = {http://adsabs.harvard.edu/abs/2011ApJ...737..103S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{VanHamme+1993,
   author = {{VanHamme}, W. },
    title = "{New limb-darkening coefficients for modeling binary star light curves }",
  journal = {\ AJ},
   eprint = {ISSN 0004-6256},
 keywords = {Binary Stars - Coefficients - Light Curve - Limb Darkening - Linear Equations - Nonlinear Equations - Stellar Models - Chemical Composition - Least Squares Method - Stellar Atmospheres},
     year = 1993,
    month = Nov,
   volume = 106,
    pages = {2096-2117},
      doi = {10.1086/116788},
   url = {http://adsabs.harvard.edu/abs/1993AJ....106.2096V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Wilson+Devinney+1971,
   author = {{Wilson}, R.~E. and {Devinney}, E.~J. },
    title = "{Realization of Accurate Close-Binary Light Curves: Application to MR Cygni}",
  journal = {\ ApJ},
     year = 1971,
    month = July,
   volume = 166,
    pages = {605-619},
      doi = {10.1086/150986},
   url = {http://adsabs.harvard.edu/abs/1971ApJ...166..605W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

